U.S. Test System with High Spatial and Temporal Resolution for Renewable Integration Studies

Planning for power systems with high penetrations of variable renewable energy requires higher spatial and temporal granularity. However, most publicly available test systems are of insufficient fidelity for developing methods and tools for high-resolution planning. This paper presents methods to construct open-access test systems of high spatial resolution to more accurately represent infrastructure and high temporal resolution to represent dynamics of demand and variable resources. To demonstrate, a high-resolution test system representing the United States is created using only publicly available data. This test system is validated by running it in a production cost model, with results compared against historical generation to ensure that they are representative. The resulting open source test system can support power system transition planning and aid in development of tools to answer questions around how best to reach decarbonization goals, using the most effective combinations of transmission expansion, renewable generation, and energy storage.

==> 04_Simulation_Platform.tex <==
\begin{figure}[ht]
\begin {center}
\includegraphics[width=3.4in]{figures/simulation_platform_block_chart.pdf}
\caption{Simulation Platform}
\label{fig:simplat_block}
\end{center}
\end{figure}

We build our simulation platform from scratch and plan to make it publicly available for open access in the near future. The platform framework consists of four components as shown in Fig \ref{fig:simplat_block}, i.e. PowerSimData, PreREISE, REISE and PostREISE. The core component is Renewable Energy Integration Simulation Engine (REISE). REISE is composed of two subcomponents, MatPower and Gurobi, i.e. a wrapper and a solver. Based on the static data provided in PowerSimData and the time-series data profiles prepared in PreREISE, the wrapper assembles the data frames and transforms the Optimal Power Flow (OPF) problem into a general optimization problem, then feeds into the solver.

The timeline to simulate a scenario of interest is as following: the user chooses a network topology and customize generator capacities and cost curves in PowerSimData, then PreREISE generates the corresponding time series data for demand, hydro, wind and solar through different methodologies at user's choice, then REISE does the heavy lift and produces the OPF results, finally PostREISE extracts the outputs and further processes the results in the analysis component. For large scale power system simulations, visualization is critical to get better insights from the results. We specifically create a visualization toolbox in Python which illustrates the outputs of the analysis component by different type of plots. We will demonstrate more details with a case study in the following section. 
